Population viewpoint on Hawkes processes

This paper focuses on a class of linear Hawkes processes with general immigrants. These are counting processes with shot noise intensity, including self-excited and externally excited patterns. For such processes, we introduce the concept of age pyramid which evolves according to immigration and births. The virtue if this approach that combines an intensity process definition and a branching representation is that the population age pyramid keeps track of all past events. This is used to compute new distribution properties for a class of linear Hawkes processes with general immigrants which generalize the popular exponential fertility function. The pathwise construction of the Hawkes process and its underlying population is also given.

==> beamenteteDynapop.tex <==
% \documentclass[11pt, xcolor=pdftex,dvipsnames,table,hidesubsections]{beamer}
% \documentclass[11pt,handout]{beamer}
\usetheme{I80new}

%==============================
\usepackage{enumerate}
\usepackage{amsmath,amssymb,array,tabularx,framed, calc,multicol}%tabls
\usepackage{amsthm}
\usepackage{wasysym}					 % pour les triangles LHD et RHD
\usepackage{verbatim}

\usepackage{empheq} 
\usepackage{parskip}  					%espace
\usepackage{setspace}					%espaceligneslides
\usepackage{comment}					%mettre en commentaire
%+++++++++++++++++++++++++++++++++++++++++++++francaisanglais
%\usepackage[francais]{babel}
\usepackage[english]{babel}
\usepackage[applemac]{inputenc}
% Texte composé avec les accents, codé dans le format "latin1" (linux) :
%\usepackage[latin1]{inputenc}

%=================================================images
\usepackage{graphicx}
%\usepackage[pdftex]{graphicx}
%\usepackage{epstopdf} permet eventuellement d'insere des images eps
%\usepackage{pgf,pgfarrows,pgfnodes,pgfautomata,pgfheaps}
\usepackage{mathrsfs}						% pour les fontmath caligraph. 		
\usepackage[controls]{animate}
\usepackage{subfigure, epsfig}  %mettre plusieurs figures dans la meme page

%\setbeamertemplate{caption}[numbered] 		%Pour numÈroter les figures
%\setbeamersize{text margin left=0.2cm,text margin right=0.2cm}
%

%\usepackage[all]{xy}

%============================================================
\usepackage{colortbl}
\usepackage{xcolor}
\usepackage{color}

%==================================================
%=======================================
\newenvironment{Frame}{\frame[allowframebreaks]}{}
\newcommand{\bFrame} {begin{Frame}}
\newcommand{\eFrame} {\end{Frame}}

\newenvironment{pframe}{\frame[plain]}{}
\newcommand{\bpframe} {begin{pframe}}
\newcommand{\epframe} {\end{pframe}}




%================equation en couleur
%\fcolorbox{violet}{i80orange!10!}{\parbox[c][0.68cm][c]{10.8cm}{
%\begin{empheq}{alignat=1}
%-\,dU_t=g(t,U_t, Z_t) dt -Z_t dW_t, \quad U_T(\xi_T)=u(\xi_T) \mbox{ for given}\>{\crouge  concave \>u}\nonumber
%{alignat=2}
%d\tU(t,y)&=&\gamma(t,-\tU_y(t,y)).dW_t+\beta(t,-\tU_y(t,y))dt \nonumber \\
%&+&\frac{1}{2} \tU_{yy}(t,y)\|\gamma_x\big(t,-\tU_y(t,y)\big)\|^2\,dt  \nonumber 
%\end{empheq}
%}
%}







%==============================================


%\usepackage{eso-pic}
%\usepackage{monster2e}
%\usepackage{tikz}
%\usepackage{layout}

%\usepackage{fancybox}
%\usepackage[absolute,showboxes,overlay]{textpos}
%\TPshowboxesfalse
%\textblockorigin{0mm}{0mm}





\def\bcomm{\begin{comment}}
\def\ecomm{\end{comment}}
%========================================================item
\def\bit{\begin{itemize}}
\def\eit{\end{itemize}}
\setbeamertemplate{itemize item}[triangle]
\setbeamertemplate{itemize subitem}[ball]


\newcommand{\rmi}{{\rm (i) $\>\>$}}
\newcommand{\rmil}{{\rm (i) $\>\>\>$}}
\newcommand{\rmii}{{\rm (ii) $\hspace{1.5mm}$}}
\newcommand{\rmiii}{{\rm (iii)$\>\>$}}
\newcommand{\rmiv}{{\rm (iv)$\>\>$}}
\newcommand{\rmv}{{\rm (v)$\>\>$}}

\def\bc{\begin{center}}
\def\ec{\end{center}}


\newcommand{\Cbullet}{{\color{DarkBlue}{\bullet}}}

%==============================================CommandeLap
\providecommand{\U}[1]{\protect\rule{.1in}{.1in}}
\newenvironment{stepenumerate}{\begin{enumerate}[<+->]}{\end{enumerate}}
\newenvironment{stepitemize}{\begin{itemize}[<+->]}{\end{itemize} }
\newenvironment{stepenumeratewithalert}{\begin{enumerate}[<+-| alert@+>]}{\end{enumerate}}
\newenvironment{stepitemizewithalert}{\begin{itemize}[<+-| alert@+>]}{\end{itemize} }
\def\bitstep{\begin{stepitemize}}
\def\eitstep{\end{stepitemize}}

%\newcommand{\mean}{\mathbb E}
%\newcommand{\meas}{\operatornamewithlimits{ess\,sup}}
%\newcommand{\amax}{\operatornamewithlimits{arg\,max}}
%\newcommand{\amin}{\operatornamewithlimits{arg\,min}}



%==============================================
%mettre des numeros aux slides

\setbeamertemplate{footline}
{
\hfill{\scriptsize{\insertframenumber/\inserttotalframenumber}}\hspace*{.5cm}
\begin{beamercolorbox}[wd=.6\paperwidth,ht=2.8ex,dp=1.125ex,leftskip=.3cm plus1fill,rightskip=.3cm]{author in head/foot}
 \usebeamerfont{author in head/foot}\insertshortauthor
  \end{beamercolorbox}%
  \begin{beamercolorbox}[wd=.4\paperwidth,ht=2.8ex,dp=1.125ex,leftskip=1.7cm,rightskip=.3cm plus1fil]{title in head/foot}%
    \usebeamerfont{title in head/foot}{UPMC,LPMA}
  \end{beamercolorbox}
  
   \vskip0pt
}




%=======couleur

%===============vert


%\newcommand{\cblue}{\color{i80vertfonce}}
\newcommand{\cgblue}{\color{i80vertfonce}}
%
\newcommand{\cbblue}{\bf \color{i80vertfonce}}
\newcommand{\cgreen}{\color{i80vertfonce}}
 \setbeamercolor{kgreen}{fg=green!50!black}
 \newcommand{\ckgreen}{\usebeamercolor[fg]{kgreen}}


\definecolor{vert1}{RGB}{133,146,66} % vert S
\definecolor{vert2}{RGB}{157,193,7} % vert S

\definecolor{Green1}{RGB}{0,63,9} %vert fonce
\definecolor{Green2}{RGB}{85,214,59}%vert qui pete
\definecolor{DarkGreen}{RGB}{8,89,34}
\definecolor{green}{rgb}{0.1,0.6,0.1}

%================bleu
\definecolor{blue}{rgb}{0.1,0,0.8}
  \setbeamercolor{bleu}{fg=blue}
  \newcommand{\cblue}{\color{blue}}
\newcommand{\cbleu}{\usebeamercolor[fg]{blue}}

\definecolor{bleu1}{RGB}{38,109,131} % bleu S
\definecolor{bleu2}{RGB}{28,70,114} % bleu S
\definecolor{MidnightBlue}{rgb}{0.1953125,0.1953125,0.796875}
\definecolor{DarkBlue1}{RGB}{15,62,142}
\definecolor{DarkBlue}{rgb}{0.1953125,0.1953125,0.796875}
\definecolor{BlueMetal}{RGB}{144,174,206}


%=========================violet/rouge
  \setbeamercolor{violet}{fg=blue!50!red}
  \newcommand{\cviolet}{\usebeamercolor[fg]{violet}}
  
  \definecolor{my_red}{rgb}{1,0,0}
  \definecolor{rouge1}{RGB}{226,0,38}  % red P
\definecolor{rouge2}{RGB}{230,68,57}  % red S
\definecolor{bordeau}{RGB}{170,15,41}

\newcommand{\cbred}{\color{titre}}
\def\cbordeau{\color{bordeau}}

\definecolor{coultitre}{rgb}{0.60,0.05,0.12}%marronrouge
\definecolor{titre}{rgb}{0.60,0.05,0.12}%marronrouge


\definecolor{orange}{rgb}{0.796875,0.1953125,0.1953125}
\definecolor{orange1}{RGB}{243,154,38}  % orange P
\definecolor{orange2}{RGB}{236,117,40}  % orange S

%=========================brun
 \setbeamercolor{brun}{fg=i80orangef!90!black!120}
   \newcommand{\cbrun}{\usebeamercolor[fg]{brun}}
   \newcommand{\crouge}{\usebeamercolor[fg]{brun}}

%=========================blanc/gris/noir
\definecolor{grey}{rgb}{0.5,0.5,0.5}
\definecolor{my_white}{rgb}{1.0,1.0,1.0}
\definecolor{gris}{RGB}{91,94,111} % gris S
\definecolor{blanc}{RGB}{255,255,255} % blanc P




\definecolor{pink}{rgb}{0.734375,0.55859375,0.55859375}
\definecolor{glauque}{rgb}{.9, .0, 0.4}
\definecolor{taupe}{RGB}{134,113,127} % taupe S
\definecolor{jaune}{RGB}{254,205,27}  % jaune P

\definecolor{Beige}{RGB}{175,118,77}
\definecolor{Beigeclair}{RGB}{244,230,221}
\definecolor{Chocolat}{RGB}{93,57,57}
\definecolor{BMD}{RGB}{93,96,153}
\newcommand{\Glauque}[1]{\textcolor{glauque}{#1}}



  
%====================================
%pour definir ses propores couleurs dans un theme
%\usecolortheme[color]{structure}
%
%le texte normal ecrit noir sur blanc
%\setbeamercolor{normal text}{fg=black,bg=white}
%\setbeamercolor{alerted text}{fg=coulalert}
%\setbeamercolor{example text}{fg=fondtitre}
%\setbeamercolor{structure}{fg=beamer@blendedblue}
%\definecolor{fondtitre}{rgb}{0.20,0.43,0.09}%vertfonce
%\definecolor{coultitre}{rgb}{0.60,0.05,0.12}%marronrouge
%\definecolor{}{rgb}{0.60,0.05,0.12}%marronrouge
%\definecolor{coulalert}{rgb}{0.80,0.05,0.10}%rougefonce

%===================================================================
\beamerboxesdeclarecolorscheme{alert}{Red}{Red!20}

\beamerboxesdeclarecolorscheme{I80new}{i80orange!150!}{red!4!i80orange!10!}

%
\beamerboxesdeclarecolorscheme{bleuvert}
{blue!50}{LimeGreen!6!}

\beamerboxesdeclarecolorscheme{marronvert}
{i80vertfonce!60}{LimeGreen!5!}


\beamerboxesdeclarecolorscheme{violet}{
bordeau!60!black!30}{violet!80!white!5}

\beamerboxesdeclarecolorscheme{vertmarron}{
PineGreen!80!black}{Maroon!10}
%
\setbeamercolor{vertclair}{fg=black,bg=yellow!7,5}

\beamerboxesdeclarecolorscheme{coultitre}{
coultitre}{Maroon!3}
%%%%%%%%%%
\setbeamertemplate{blocks}[rounded][shadow=TRUE]

%====================================



%========================================
\def\vp1{\vspace*{1mm}}
\def\vp2{\vspace*{2mm}}
\def\vp3{\vspace*{3mm}}
\def\vp5{\vspace*{5mm}}
\def\vp7{\vspace*{7mm}}


\def\C{{\mathbb C}}
\def\D{{\mathbb D}}
\def\E{\mathbb{E}}
\def\LL{{\mathbb L}}
\def\N{{\mathbb N}}
\def\Pr{\mathbb{P}}
\def\P{{\mathbb P}}
\def\Q{{\mathbb Q}}
\def\R{{\mathbb R}}
%
\def\cal{\mathcal}

\def\cC{{ \mathcal C}}
\def\cF{{ \mathcal F}}
\def\K{{\cal K}}
\def\cK{{\cal K}}
\def\IK{{\cal IK}}
%
\def\cL{{\cal L}}
\def\cI{{\cal I}}
\def\cM{{\mathcal M}}
\def\cO{{\cal O}}
\def\O{{\cal O}}
%
\def\cP{{\cal P}}
%
\def\X{{ \mathcal X}}
\def\cX{{ \mathcal X}}
%
\def\Y{{\mathcal Y}}
\def\cY{{\mathcal Y}}
%
\def\Ac{{\cal A}}
\def\Bc{{\cal B}}
\def\Cc{{\cal C}}
\def\Dc{{\cal D}}
\def\Ec{{\cal E}}
\def\Fc{{\cal F}}
\def\Gc{{\cal G}}
\def\Hc{{\cal H}}
\def\Ic{{\cal I}}
\def\Jc{{\cal J}}
\def\Kc{{\cal K}}
\def\Lc{{\cal L}}
\def\Mc{{\cal M}}
\def\Nc{{\cal N}}
\def\Oc{{\cal O}}
\def\Pc{{\cal P}}
\def\Pcb{\overline{\Pc}}
\def\Pch{\widehat{\Pc}}
\def\Qc{{\cal Q}}
\def\Rc{{\cal R}}
\def\Sc{{\cal S}}
\def\Tc{{\cal T}}
\def\Uc{{\cal U}}
\def\Vc{{\cal V}}
\def\Xc{{\cal X}}
\def\Yc{{\cal Y}}
\def\Zc{{\cal Z}}

%%

\def\sQ{\mathsf {Q}}


\def\I{{\mathbf I}}
\def\bI{{\mathbf I}}

\def\Lb{{\bar L}}
\def\Pb{\overline{\P}}
\def\Qb{\overline{\Q}}
\def\Rb{\overline{\R}}
\def\Rcb{{\overline{\Rc}}}
\def\Db{\overline{D}}
\def\Dbb{\overline{\D}}
\def\Dcb{\overline{\Dc}}

\def\Ab{\overline{A}}
\def\Mb{\overline{M}}
\def\oK{{\overline{\mathcal K}}}
\def\tK{{\overline {\mathcal K}}}
\newcommand{\oU} {{\overline {U}}}
\newcommand{\oV} {{\overline {V}}}
\newcommand{\oX} {{\overline {X}}}
\newcommand{\oZ} {{\overline {Z}}}
\def \Ecb{\overline{\Ec}}

\def\xb{\mathbf{x}}
\def \wh{ \hat{\w}}
\def \mh{\hat{m}}
\def \omb{ \bar{\om}}
\def \Acb{ \overline{\Ac}}
\def \Tcb{ \overline{\Tc}}
\def \eps{\varepsilon}
\def \Sig{\Sigma}
\def \Fcb{\overline{{\cal F}}}
\def \Fbb{\overline{\mathbb{F}}}
\def\Fch{\widehat{\Fc}}

\def\Rct{\tilde{\Rc}}
\def\Rch{\widehat{\Rc}}
\def \Ph{\widehat{\P}}
\def \tauh{\hat{\tau}}
\def \taub{\bar{\tau}}

%
\def\tG{\tilde{\gamma}}
\def\tp{{\tilde \pi}}
\def\tU{{\tilde U}}
\def\tu{{\tilde u}}
\def\tK{{\tilde {\mathcal K}}}


\newcommand{\GP}{{\mathscr P}}
\newcommand{\GV}{{\mathscr V}}
\newcommand{\GY}{{\mathscr Y}}
\newcommand{\GX}{{\mathscr X}}
%
\def\cR{{\cal R}^{a,c}}
\def\sigR{{\cal R}^\sigma}
\def\sR{\text{{\tiny${\cal R}$}}}
\def\sigoR{{\cal R}^{\sigma,\perp}}




\def\Var{\mathop{\mathrm{Var}}}
\def\neg{\negthickspace \negthickspace}
\def\PX{{\mathbb X}^+ }
%\def\GK{{\mathfrak  Y}}
\def\t{{\texttt{t}}}


\def\Ha{$\mathbf{H_1}$ }
\def\Hb{$\mathbf{H_2}$ }

%%% greek %%%%
\def \a{\alpha}
\def\lam{\lambda}
\def\Lam{\Lambda}

\def \O{\Omega}
\def \Om{\Omega}
\def \Ob{\overline{\Omega}}
\def \Omb{\overline{\Om}}
\def \Omh{\widehat{\Om}}

\def \o{\omega}
\def \om{\o}
\def \omh{ \hat{\om}}
\def\psib{\overline{\psi}}
\def\tsig{{\tilde \sigma}}
%===================================grecqu



\def\sigoR{{\cal R}^{\sigma,\perp}}
\def\Ha{$\mathbf{H_1}$ }
\def\Hb{$\mathbf{H_2}$ }



\def\PX{{\mathbb X}^+ }
%\def\GK{{\mathfrak  Y}}
\def\tsig{{\tilde \sigma}}
\def\t{{\texttt{t}}}


\def\ind{{\bf 1}}
\def\demi{\frac{1}{2}}


\def\t{{\texttt{t}}}
\def\logit{\,{\text{logit}}\,}
\def\x{\times}
\def\ox{\otimes}

\newcommand{\mean}{\mathbb E}

\newcommand{\essup}{\operatornamewithlimits{ess\,sup}}
\newcommand{\argmax}{\operatornamewithlimits{arg\,max}}
\newcommand{\argmin}{\operatornamewithlimits{arg\,min}}






\newcommand{\edoc} {\end{document}}

  % \setstretch{1.15}
%\setlength{\parskip}{4pt plus 1pt minus 1pt}

%\graphicspath{{./graphesmortalite/}}

%Ajouté par Alexandre le 13/05/13
\def\du{\,{\partial \over \partial u}}
\def\da{\,{\partial \over \partial a}}
\def\ds{\,{\partial \over \partial s}}
\def\1{{\mathbf{1}}}
\def\d{{\mathrm{d}}}
\def\M{{\mathcal{M}}}
\def\F{{\mathcal{F}}}





==> beamenteteLiverpool2013.tex <==
% \documentclass[11pt, xcolor=pdftex,dvipsnames,table,hidesubsections]{beamer}
% \documentclass[11pt,handout]{beamer}
\usetheme{I80new}

%==============================
\usepackage{enumerate}
\usepackage{amsmath,amssymb,array,tabularx,framed, calc,multicol}%tabls
\usepackage{amsthm}
\usepackage{wasysym}					 % pour les triangles LHD et RHD
\usepackage{verbatim}

\usepackage{empheq} 
\usepackage{parskip}  					%espace
\usepackage{setspace}					%espaceligneslides
\usepackage{comment}					%mettre en commentaire
%+++++++++++++++++++++++++++++++++++++++++++++francaisanglais
%\usepackage[francais]{babel}
\usepackage[english]{babel}
\usepackage[applemac]{inputenc}
% Texte composé avec les accents, codé dans le format "latin1" (linux) :
%\usepackage[latin1]{inputenc}

%=================================================images
\usepackage{graphicx}
%\usepackage[pdftex]{graphicx}
%\usepackage{epstopdf} permet eventuellement d'insere des images eps
%\usepackage{pgf,pgfarrows,pgfnodes,pgfautomata,pgfheaps}
\usepackage{mathrsfs}						% pour les fontmath caligraph. 		
\usepackage[controls]{animate}
\usepackage{subfigure, epsfig}  %mettre plusieurs figures dans la meme page

%\setbeamertemplate{caption}[numbered] 		%Pour numÈroter les figures
%\setbeamersize{text margin left=0.2cm,text margin right=0.2cm}
%

%\usepackage[all]{xy}

%============================================================
\usepackage{colortbl}
\usepackage{xcolor}
\usepackage{color}

%==================================================
%=======================================
\newenvironment{Frame}{\frame[allowframebreaks]}{}
\newcommand{\bFrame} {begin{Frame}}
\newcommand{\eFrame} {\end{Frame}}

\newenvironment{pframe}{\frame[plain]}{}
\newcommand{\bpframe} {begin{pframe}}
\newcommand{\epframe} {\end{pframe}}




%================equation en couleur
%\fcolorbox{violet}{i80orange!10!}{\parbox[c][0.68cm][c]{10.8cm}{
%\begin{empheq}{alignat=1}
%-\,dU_t=g(t,U_t, Z_t) dt -Z_t dW_t, \quad U_T(\xi_T)=u(\xi_T) \mbox{ for given}\>{\crouge  concave \>u}\nonumber
%{alignat=2}
%d\tU(t,y)&=&\gamma(t,-\tU_y(t,y)).dW_t+\beta(t,-\tU_y(t,y))dt \nonumber \\
%&+&\frac{1}{2} \tU_{yy}(t,y)\|\gamma_x\big(t,-\tU_y(t,y)\big)\|^2\,dt  \nonumber 
%\end{empheq}
%}
%}







%==============================================


%\usepackage{eso-pic}
%\usepackage{monster2e}
%\usepackage{tikz}
%\usepackage{layout}

%\usepackage{fancybox}
%\usepackage[absolute,showboxes,overlay]{textpos}
%\TPshowboxesfalse
%\textblockorigin{0mm}{0mm}





\def\bcomm{\begin{comment}}
\def\ecomm{\end{comment}}
%========================================================item
\def\bit{\begin{itemize}}
\def\eit{\end{itemize}}
\setbeamertemplate{itemize item}[triangle]
\setbeamertemplate{itemize subitem}[ball]


\newcommand{\rmi}{{\rm (i) $\>\>$}}
\newcommand{\rmil}{{\rm (i) $\>\>\>$}}
\newcommand{\rmii}{{\rm (ii) $\hspace{1.5mm}$}}
\newcommand{\rmiii}{{\rm (iii)$\>\>$}}
\newcommand{\rmiv}{{\rm (iv)$\>\>$}}
\newcommand{\rmv}{{\rm (v)$\>\>$}}

\def\bc{\begin{center}}
\def\ec{\end{center}}


\newcommand{\Cbullet}{{\color{DarkBlue}{\bullet}}}

%==============================================CommandeLap
\providecommand{\U}[1]{\protect\rule{.1in}{.1in}}
\newenvironment{stepenumerate}{\begin{enumerate}[<+->]}{\end{enumerate}}
\newenvironment{stepitemize}{\begin{itemize}[<+->]}{\end{itemize} }
\newenvironment{stepenumeratewithalert}{\begin{enumerate}[<+-| alert@+>]}{\end{enumerate}}
\newenvironment{stepitemizewithalert}{\begin{itemize}[<+-| alert@+>]}{\end{itemize} }
\def\bitstep{\begin{stepitemize}}
\def\eitstep{\end{stepitemize}}

%\newcommand{\mean}{\mathbb E}
%\newcommand{\meas}{\operatornamewithlimits{ess\,sup}}
%\newcommand{\amax}{\operatornamewithlimits{arg\,max}}
%\newcommand{\amin}{\operatornamewithlimits{arg\,min}}



%==============================================
%mettre des numeros aux slides

\setbeamertemplate{footline}
{
\hfill{\scriptsize{\insertframenumber/\inserttotalframenumber}}\hspace*{.5cm}
\begin{beamercolorbox}[wd=.6\paperwidth,ht=2.8ex,dp=1.125ex,leftskip=.3cm plus1fill,rightskip=.3cm]{author in head/foot}
 \usebeamerfont{author in head/foot}\insertshortauthor
  \end{beamercolorbox}%
  \begin{beamercolorbox}[wd=.4\paperwidth,ht=2.8ex,dp=1.125ex,leftskip=1.7cm,rightskip=.3cm plus1fil]{title in head/foot}%
    \usebeamerfont{title in head/foot}{UPMC,LPMA}
  \end{beamercolorbox}
  
   \vskip0pt
}




%=======couleur

%===============vert


%\newcommand{\cblue}{\color{i80vertfonce}}
\newcommand{\cgblue}{\color{i80vertfonce}}
%
\newcommand{\cbblue}{\bf \color{i80vertfonce}}
\newcommand{\cgreen}{\color{i80vertfonce}}
 \setbeamercolor{kgreen}{fg=green!50!black}
 \newcommand{\ckgreen}{\usebeamercolor[fg]{kgreen}}


\definecolor{vert1}{RGB}{133,146,66} % vert S
\definecolor{vert2}{RGB}{157,193,7} % vert S

\definecolor{Green1}{RGB}{0,63,9} %vert fonce
\definecolor{Green2}{RGB}{85,214,59}%vert qui pete
\definecolor{DarkGreen}{RGB}{8,89,34}
\definecolor{green}{rgb}{0.1,0.6,0.1}

%================bleu
\definecolor{blue}{rgb}{0.1,0,0.8}
  \setbeamercolor{bleu}{fg=blue}
  \newcommand{\cblue}{\color{blue}}
\newcommand{\cbleu}{\usebeamercolor[fg]{blue}}

\definecolor{bleu1}{RGB}{38,109,131} % bleu S
\definecolor{bleu2}{RGB}{28,70,114} % bleu S
\definecolor{MidnightBlue}{rgb}{0.1953125,0.1953125,0.796875}
\definecolor{DarkBlue1}{RGB}{15,62,142}
\definecolor{DarkBlue}{rgb}{0.1953125,0.1953125,0.796875}
\definecolor{BlueMetal}{RGB}{144,174,206}


%=========================violet/rouge
  \setbeamercolor{violet}{fg=blue!50!red}
  \newcommand{\cviolet}{\usebeamercolor[fg]{violet}}
  
  \definecolor{my_red}{rgb}{1,0,0}
  \definecolor{rouge1}{RGB}{226,0,38}  % red P
\definecolor{rouge2}{RGB}{230,68,57}  % red S
\definecolor{bordeau}{RGB}{170,15,41}

\newcommand{\cbred}{\color{titre}}
\def\cbordeau{\color{bordeau}}

\definecolor{coultitre}{rgb}{0.60,0.05,0.12}%marronrouge
\definecolor{titre}{rgb}{0.60,0.05,0.12}%marronrouge


\definecolor{orange}{rgb}{0.796875,0.1953125,0.1953125}
\definecolor{orange1}{RGB}{243,154,38}  % orange P
\definecolor{orange2}{RGB}{236,117,40}  % orange S

%=========================brun
 \setbeamercolor{brun}{fg=i80orangef!90!black!120}
   \newcommand{\cbrun}{\usebeamercolor[fg]{brun}}
   \newcommand{\crouge}{\usebeamercolor[fg]{brun}}

%=========================blanc/gris/noir
\definecolor{grey}{rgb}{0.5,0.5,0.5}
\definecolor{my_white}{rgb}{1.0,1.0,1.0}
\definecolor{gris}{RGB}{91,94,111} % gris S
\definecolor{blanc}{RGB}{255,255,255} % blanc P




\definecolor{pink}{rgb}{0.734375,0.55859375,0.55859375}
\definecolor{glauque}{rgb}{.9, .0, 0.4}
\definecolor{taupe}{RGB}{134,113,127} % taupe S
\definecolor{jaune}{RGB}{254,205,27}  % jaune P

\definecolor{Beige}{RGB}{175,118,77}
\definecolor{Beigeclair}{RGB}{244,230,221}
\definecolor{Chocolat}{RGB}{93,57,57}
\definecolor{BMD}{RGB}{93,96,153}
\newcommand{\Glauque}[1]{\textcolor{glauque}{#1}}



  
%====================================
%pour definir ses propores couleurs dans un theme
%\usecolortheme[color]{structure}
%
%le texte normal ecrit noir sur blanc
%\setbeamercolor{normal text}{fg=black,bg=white}
%\setbeamercolor{alerted text}{fg=coulalert}
%\setbeamercolor{example text}{fg=fondtitre}
%\setbeamercolor{structure}{fg=beamer@blendedblue}
%\definecolor{fondtitre}{rgb}{0.20,0.43,0.09}%vertfonce
%\definecolor{coultitre}{rgb}{0.60,0.05,0.12}%marronrouge
%\definecolor{}{rgb}{0.60,0.05,0.12}%marronrouge
%\definecolor{coulalert}{rgb}{0.80,0.05,0.10}%rougefonce

%===================================================================
\beamerboxesdeclarecolorscheme{alert}{Red}{Red!20}

\beamerboxesdeclarecolorscheme{I80new}{i80orange!150!}{red!4!i80orange!10!}

%
\beamerboxesdeclarecolorscheme{bleuvert}
{blue!50}{LimeGreen!6!}

\beamerboxesdeclarecolorscheme{marronvert}
{i80vertfonce!60}{LimeGreen!5!}


\beamerboxesdeclarecolorscheme{violet}{
bordeau!60!black!30}{violet!80!white!5}

\beamerboxesdeclarecolorscheme{vertmarron}{
PineGreen!80!black}{Maroon!10}
%
\setbeamercolor{vertclair}{fg=black,bg=yellow!7,5}

\beamerboxesdeclarecolorscheme{coultitre}{
coultitre}{Maroon!3}
%%%%%%%%%%
\setbeamertemplate{blocks}[rounded][shadow=TRUE]

%====================================



%========================================
\def\vp1{\vspace*{1mm}}
\def\vp2{\vspace*{2mm}}
\def\vp3{\vspace*{3mm}}
\def\vp5{\vspace*{5mm}}
\def\vp7{\vspace*{7mm}}


\def\C{{\mathbb C}}
\def\D{{\mathbb D}}
\def\E{\mathbb{E}}
\def\LL{{\mathbb L}}
\def\N{{\mathbb N}}
\def\Pr{\mathbb{P}}
\def\P{{\mathbb P}}
\def\Q{{\mathbb Q}}
\def\R{{\mathbb R}}
%
\def\cal{\mathcal}

\def\cC{{ \mathcal C}}
\def\cF{{ \mathcal F}}
\def\K{{\cal K}}
\def\cK{{\cal K}}
\def\IK{{\cal IK}}
%
\def\cL{{\cal L}}
\def\cI{{\cal I}}
\def\cM{{\mathcal M}}
\def\cO{{\cal O}}
\def\O{{\cal O}}
%
\def\cP{{\cal P}}
%
\def\X{{ \mathcal X}}
\def\cX{{ \mathcal X}}
%
\def\Y{{\mathcal Y}}
\def\cY{{\mathcal Y}}
%
\def\Ac{{\cal A}}
\def\Bc{{\cal B}}
\def\Cc{{\cal C}}
\def\Dc{{\cal D}}
\def\Ec{{\cal E}}
\def\Fc{{\cal F}}
\def\Gc{{\cal G}}
\def\Hc{{\cal H}}
\def\Ic{{\cal I}}
\def\Jc{{\cal J}}
\def\Kc{{\cal K}}
\def\Lc{{\cal L}}
\def\Mc{{\cal M}}
\def\Nc{{\cal N}}
\def\Oc{{\cal O}}
\def\Pc{{\cal P}}
\def\Pcb{\overline{\Pc}}
\def\Pch{\widehat{\Pc}}
\def\Qc{{\cal Q}}
\def\Rc{{\cal R}}
\def\Sc{{\cal S}}
\def\Tc{{\cal T}}
\def\Uc{{\cal U}}
\def\Vc{{\cal V}}
\def\Xc{{\cal X}}
\def\Yc{{\cal Y}}
\def\Zc{{\cal Z}}

%%

\def\sQ{\mathsf {Q}}


\def\I{{\mathbf I}}
\def\bI{{\mathbf I}}

\def\Lb{{\bar L}}
\def\Pb{\overline{\P}}
\def\Qb{\overline{\Q}}
\def\Rb{\overline{\R}}
\def\Rcb{{\overline{\Rc}}}
\def\Db{\overline{D}}
\def\Dbb{\overline{\D}}
\def\Dcb{\overline{\Dc}}

\def\Ab{\overline{A}}
\def\Mb{\overline{M}}
\def\oK{{\overline{\mathcal K}}}
\def\tK{{\overline {\mathcal K}}}
\newcommand{\oU} {{\overline {U}}}
\newcommand{\oV} {{\overline {V}}}
\newcommand{\oX} {{\overline {X}}}
\newcommand{\oZ} {{\overline {Z}}}
\def \Ecb{\overline{\Ec}}

\def\xb{\mathbf{x}}
\def \wh{ \hat{\w}}
\def \mh{\hat{m}}
\def \omb{ \bar{\om}}
\def \Acb{ \overline{\Ac}}
\def \Tcb{ \overline{\Tc}}
\def \eps{\varepsilon}
\def \Sig{\Sigma}
\def \Fcb{\overline{{\cal F}}}
\def \Fbb{\overline{\mathbb{F}}}
\def\Fch{\widehat{\Fc}}

\def\Rct{\tilde{\Rc}}
\def\Rch{\widehat{\Rc}}
\def \Ph{\widehat{\P}}
\def \tauh{\hat{\tau}}
\def \taub{\bar{\tau}}

%
\def\tG{\tilde{\gamma}}
\def\tp{{\tilde \pi}}
\def\tU{{\tilde U}}
\def\tu{{\tilde u}}
\def\tK{{\tilde {\mathcal K}}}


\newcommand{\GP}{{\mathscr P}}
\newcommand{\GV}{{\mathscr V}}
\newcommand{\GY}{{\mathscr Y}}
\newcommand{\GX}{{\mathscr X}}
%
\def\cR{{\cal R}^{a,c}}
\def\sigR{{\cal R}^\sigma}
\def\sR{\text{{\tiny${\cal R}$}}}
\def\sigoR{{\cal R}^{\sigma,\perp}}




\def\Var{\mathop{\mathrm{Var}}}
\def\neg{\negthickspace \negthickspace}
\def\PX{{\mathbb X}^+ }
%\def\GK{{\mathfrak  Y}}
\def\t{{\texttt{t}}}


\def\Ha{$\mathbf{H_1}$ }
\def\Hb{$\mathbf{H_2}$ }

%%% greek %%%%
\def \a{\alpha}
\def\lam{\lambda}
\def\Lam{\Lambda}

\def \O{\Omega}
\def \Om{\Omega}
\def \Ob{\overline{\Omega}}
\def \Omb{\overline{\Om}}
\def \Omh{\widehat{\Om}}

\def \o{\omega}
\def \om{\o}
\def \omh{ \hat{\om}}
\def\psib{\overline{\psi}}
\def\tsig{{\tilde \sigma}}
%===================================grecqu



\def\sigoR{{\cal R}^{\sigma,\perp}}
\def\Ha{$\mathbf{H_1}$ }
\def\Hb{$\mathbf{H_2}$ }



\def\PX{{\mathbb X}^+ }
%\def\GK{{\mathfrak  Y}}
\def\tsig{{\tilde \sigma}}
\def\t{{\texttt{t}}}


\def\ind{{\bf 1}}
\def\demi{\frac{1}{2}}


\def\t{{\texttt{t}}}
\def\logit{\,{\text{logit}}\,}
\def\x{\times}
\def\ox{\otimes}

\newcommand{\mean}{\mathbb E}

\newcommand{\essup}{\operatornamewithlimits{ess\,sup}}
\newcommand{\argmax}{\operatornamewithlimits{arg\,max}}
\newcommand{\argmin}{\operatornamewithlimits{arg\,min}}






\newcommand{\edoc} {\end{document}}

  % \setstretch{1.15}
%\setlength{\parskip}{4pt plus 1pt minus 1pt}

%\graphicspath{{./graphesmortalite/}}










